Observed Timescales of Stellar Feedback in Star-Forming, Low-Mass Galaxies

Understanding the timescales of atomic gas turbulence is crucial to understanding the interplay between star formation and the interstellar medium (ISM). To investigate the timescales of turbulence low-mass galaxies ($10^{6.8}<M_\odot<10^9$), this study combines temporally resolved star formation histories (SFHs) -- derived from color-magnitude diagrams -- with kinematic data of the atomic and ionized hydrogen in a large sample of nearby, star-forming, low-mass galaxies. To best understand the timescales involved, SFHs and gas kinematics were analyzed in 400$\times$400 parsec regions to capture the local impacts of star formation. No strong correlation was found between the ionized gas velocity dispersion and the star formation activity over the past 5-500 Myr. In contrast, a consistent and significant correlation between the atomic hydrogen turbulence measures and the star formation activity t$\geq$100 Myr ago was identified. This correlation suggests the star formation activity and atomic gas are coupled on this timescale. This connection between star-formation activity $>$100 Myr ago, and the HI turbulence properties, may be related to the time scales over which turbulence decays in the ISM. Additionally, the results demonstrate a possible difference in the global and local turbulence properties of low-mass galaxies.

==> Hunter_2025_PhD_paper_submit_3_/Scrapped.tex <==
%An accurate understanding of how galaxies evolve is fundamental to modeling individual galaxies to the large-scale universe and individual galaxies.  Stellar feedback drives turbulence in the interstellar medium (ISM) (, and is a key process impacting the evolution of galaxies, as it affects galaxies across different physical scales and timescales. 

%In prior observational work, using integrated light star formation rates, there is evidence of a clear correlation between star formation and ISM turbulence.  \cite{Moiseev15} demonstrated that the ionized gas velocity dispersions are a result of thermal motions and energy output by current star formation activity. Additionally, \cite{Joung09,Tamburro09,Stilp13c} present indications that the atomic gas turbulence is associated with star formation at high star formation rate (SFR) surface densities. However, the spatial correlation between star formation and changes in the energy density of the ISM may not be so obvious. \cite{Hunter21} and \cite{Elmegreen22} cross-correlated the kinetic energy density of the neutral ISM with the star formation rate (SFR) surface density for LITTLE THINGS \citep{LTHINGS} and THINGS \citep{things} respectively and found no correspondence. From this work, they concluded energy from stellar feedback has little impact on \hi turbulence at large scales and primarily disrupts molecular gas clouds.  

%By utilizing time-resolved star formation histories (SFHs), \cite{Stilp13b} identified a correlation between the globally averaged \hi turbulence and star formation activity 30-40 Myr ago. Further work in Paper I and II (here after Papers I and II)  utilizing time-resolved SFHs of five low-mass galaxies revealed a correlation between turbulence in the atomic gas and star formation $\sim$100 Myr ago on local scales. As discussed in \cite{LCH_2022, LCH_2023}, the timescales associated with local measures of turbulence appears to be different than those measured on global scales. The difference in the observed correlation timescales may indicate that there are differences between the local and global turbulence properties of galaxies.

%This observed correlation between past star formation activity and current turbulence in the ISM may be related to the dissipation timescale of the atomic gas. The dissipation of energy in atomic gas is key to understanding the processes that drive turbulence. The dissipation timescale can rule out energy sources based on the required energy and input efficiencies necessary to maintain the observed turbulence.  For example, for thin disks with modest velocity dispersions, the dissipation timescale for atomic gas has been approximated as 5-15 Myr in estimating the ability for supernovae (SNe) energy input to drive turbulence (e.g., \citealt{Tamburro09,Stilp13c,Utomo19}).  This approximation requires a SNe energy input efficiency of nearly 100\% or above, implying turbulence must be driven by additional energy sources. In contrast, observational and simulation work have demonstrated that the dissipation timescale may be on the scale of $\sim$100 Myr (e.g., \citealt{Bacchini20a,Orr2020}). This longer dissipation timescale aligns with the few to ten percent efficiencies for the transfer of energy from SNe to the atomic gas found in simulations (e.g., \citealt{Thornton98,Martizzi16,Fierlinger16}).   The observations in Paper I and II of a correlation timescale between the local star formation 100 Myr ago and the current atomic gas support this evidence of longer dissipation timescales.  Dissipation timescales of $\sim$100 Myr imply that stellar feedback energy input at lower efficiencies could be the primary driver of the observed turbulence.

%The results presented in this paper builds on the earlier work of Papers I and II expanding the sample to 26 galaxies. This sample covers 2 orders of magnitude in stellar mass (from 6.92 to 9.05 log(M$_\odot$)), far UV star formation rate (from -3.01 to -0.7 log(M$_\odot$ yr$^{-1}$)), and \hi mass (from 7.00 to 9.21 log(M$_\odot$)). This sample of 26 galaxies was selected to explore further the differences between global and local turbulence properties, and the impact of galactic properties on the feedback timescale. Section \ref{obs_c5} discusses the data used in this study from the Very Large Array (VLA\footnote{The VLA is operated by the NRAO, which is a facility of the National Science Foundation operated under cooperative agreement by Associated Universities, Inc.}), \textit{Hubble Space Telescope (HST)}, and WIYN\footnote{The WIYN Observatory is a joint facility of the NSF's National Optical-Infrared Astronomy Research Laboratory, Indiana University, the University of Wisconsin-Madison, Pennsylvania State University, the University of Missouri, the University of California-Irvine, and Purdue University. } 3.5m telescope, and Section \ref{Methods_c5} summarizes the methods detailed in Paper I and II for determining the SFHs and measuring the turbulence of the atomic and ionized gas.  Section \ref{halpha_res_c5} presents the H$\alpha$ results, Sections \ref{local_time_c5} and \ref{sec:equal} present the results for the \hi on the 400 pc scale, and Section \ref{sec:discussion_ch5} discusses the implications of these results.  Section \ref{global_time_c5} presents the global timescale results. Section \ref{conclusions_c5} summarizes the results and conclusions.

The SFHs were derived from observations of resolved stellar populations taken by \textit{HST} with either the Advanced Camera for Surveys instrument (\citealt{ACS}) or the Wide Field Planetary Camera 2 instrument (\citealt{WFPC2}).  Details of the observations are listed in Table  \ref{table:HST_obs_ch5}.  The ACS observations (202"$\times$202" field of view,  pixel scale of 0.05" pixel$^{-1}$) were taken with the camera's F814W I filter and at least one of the F606W V filter, F555W V filter, or F475W g filter. The WFPC2 observations were taken with the F814W I filter and either the F606W V filter or F555W V filter.  The WFPC2 instrument has three 800$\times$800 pixel wide field CCDs, with a 0.1" pixel $^{-1}$ pixel scale, and a 800$\times$800 pixel planetary camera CCD with a 0.05" pixel $^{-1}$ pixel scale. 

The optical imaging was processed in an identical manner to STARBIRDS \citep{McQuinn15a} and to match the processing in Paper I and II. A summary of the data reduction is provided here and the reader is referred to \cite{McQuinn10a} for a detailed description. Photometry was performed with the software DOLPHOT, optimized for the ACS and WFPC2 instruments, on the pipeline processed, charge transfer efficiency corrected images \citep{Dolphin00,Dolphot}. The photometry was filtered to include well-recovered point sources with the same quality cuts on signal-to-noise-ratios, crowding conditions, and sharpness parameters as applied in STARBIRDS. Artificial star tests were run on the individual images to measure the completeness of the stellar catalogs. As the derivation of the SFHs require a well-measured completeness function, $\sim5-6$ million artificial star tests were ran over each field of view, ensuring sufficient numbers of stars per individual region in the analysis.  

 %These estimates range from twice the disk scale heights of the galaxies (200-600 pc for dwarf galaxies measured in \cite{Patra20,Bacchini20b}), to an estimated driving scale of 2 kpc, (which is supported by \cite{Chepurnov15} who determined a 2.3 kpc turbulence driving scale from the velocity power spectrum of the SMC) and driving scales as large as 6 kpc have been predicted in simulations of dwarf galaxies \citep{Dib05}.  
 
 
%a clear correlation was evident across between the star formation at a specific time and nearly all \hi turbulence measures --100–200 Myr in Paper I for four low-mass galaxies, and in Paper II for Holmberg II.    
%In Papers I and II, a clear correlation was evident across between the star formation at a specific time and nearly all \hi turbulence measures --100–200 Myr in Paper I for four low-mass galaxies, and 70–140 Myr in Paper II for Holmberg II.  

%For the total sample, a large portion of the regions are located towards the outskirts of the galaxies. These regions have lower \hi column densities and historically have less star formation. Additionally, such regions tend to be the same regions with low current velocity dispersions. These regions can be seen on the outskirts of galaxies in Figures \ref{07843_frame} through \ref{92403_frame}. The analysis presented in the previous papers did not include significant numbers of regions in the outskirts of galaxies. In \LCHI, regions were required to have $>$50 blue stars and this blue star cut excluded the outer regions with low current star formation rates and gas masses.  In \LCHII, the HST footprint for Holmberg II does not cover the outer \hi extent of the galaxy. To illustrate the issue, in Figure \ref{sfrvhi_8.7} there is a large clustering of points with low star formation rates between 500 Myr to 14 Gyr ago and with velocity dispersions $\leq$15 km/s. This clustering appears to drive the possible correlation between the \hi velocity dispersions and the SFR in the oldest time bin. A reanalysis of the total sample with the blue star cuts in Sections \ref{blue_anal} removes many of these outer regions and shifts the peak of the correlation timescale. 


%Due to the lack of a clear correlation timescale between the SFHs and the velocity dispersions, the full sample of galaxies was re-analyzed focusing on the regions with indications of recent star formation activity.  As discussed in Paper I, the proof-of-concept analysis of four galaxies only included regions if they contained at least 50 young stars to ensure well-constrained recent SFHs.  However, these cuts were found to remove large numbers of regions of interest with star formation in the past 500 Myr. The subsequent analysis of Holmberg II discussed in Paper II did not include this cut. For the full sample, not making a cut results in the inclusion of many regions with low stellar mass, low \hi mass, and low velocity dispersion.  For some galaxies, imposing the cuts removes $\sim$10\% of the regions, with a negligible impact on the final analysis. For Holmberg II, the cut removes 13 out of 125 regions, and has no impact on the results.  However, for IC 2574, this cut removes nearly half the regions, going from 236 to 126 regions.   For the full sample 556 regions include the minimum number of blue stars. % The differences in the regions' SFHs can be seen in in Figures \ref{5666_SFH} and \ref{5666_SFH_blue}. The blue star cut removes many regions with high \hi velocity dispersions, as the blue star cut removes a prominent area of high velocity dispersion in the South of the galaxy (see Figure \ref{56663_frame}), as well as other smaller areas of high velocity dispersion. 

==> Scrapped.tex <==
%An accurate understanding of how galaxies evolve is fundamental to modeling individual galaxies to the large-scale universe and individual galaxies.  Stellar feedback drives turbulence in the interstellar medium (ISM) (, and is a key process impacting the evolution of galaxies, as it affects galaxies across different physical scales and timescales. 

%In prior observational work, using integrated light star formation rates, there is evidence of a clear correlation between star formation and ISM turbulence.  \cite{Moiseev15} demonstrated that the ionized gas velocity dispersions are a result of thermal motions and energy output by current star formation activity. Additionally, \cite{Joung09,Tamburro09,Stilp13c} present indications that the atomic gas turbulence is associated with star formation at high star formation rate (SFR) surface densities. However, the spatial correlation between star formation and changes in the energy density of the ISM may not be so obvious. \cite{Hunter21} and \cite{Elmegreen22} cross-correlated the kinetic energy density of the neutral ISM with the star formation rate (SFR) surface density for LITTLE THINGS \citep{LTHINGS} and THINGS \citep{things} respectively and found no correspondence. From this work, they concluded energy from stellar feedback has little impact on \hi turbulence at large scales and primarily disrupts molecular gas clouds.  

%By utilizing time-resolved star formation histories (SFHs), \cite{Stilp13b} identified a correlation between the globally averaged \hi turbulence and star formation activity 30-40 Myr ago. Further work in Paper I and II (here after Papers I and II)  utilizing time-resolved SFHs of five low-mass galaxies revealed a correlation between turbulence in the atomic gas and star formation $\sim$100 Myr ago on local scales. As discussed in \cite{LCH_2022, LCH_2023}, the timescales associated with local measures of turbulence appears to be different than those measured on global scales. The difference in the observed correlation timescales may indicate that there are differences between the local and global turbulence properties of galaxies.

%This observed correlation between past star formation activity and current turbulence in the ISM may be related to the dissipation timescale of the atomic gas. The dissipation of energy in atomic gas is key to understanding the processes that drive turbulence. The dissipation timescale can rule out energy sources based on the required energy and input efficiencies necessary to maintain the observed turbulence.  For example, for thin disks with modest velocity dispersions, the dissipation timescale for atomic gas has been approximated as 5-15 Myr in estimating the ability for supernovae (SNe) energy input to drive turbulence (e.g., \citealt{Tamburro09,Stilp13c,Utomo19}).  This approximation requires a SNe energy input efficiency of nearly 100\% or above, implying turbulence must be driven by additional energy sources. In contrast, observational and simulation work have demonstrated that the dissipation timescale may be on the scale of $\sim$100 Myr (e.g., \citealt{Bacchini20a,Orr2020}). This longer dissipation timescale aligns with the few to ten percent efficiencies for the transfer of energy from SNe to the atomic gas found in simulations (e.g., \citealt{Thornton98,Martizzi16,Fierlinger16}).   The observations in Paper I and II of a correlation timescale between the local star formation 100 Myr ago and the current atomic gas support this evidence of longer dissipation timescales.  Dissipation timescales of $\sim$100 Myr imply that stellar feedback energy input at lower efficiencies could be the primary driver of the observed turbulence.

%The results presented in this paper builds on the earlier work of Papers I and II expanding the sample to 26 galaxies. This sample covers 2 orders of magnitude in stellar mass (from 6.92 to 9.05 log(M$_\odot$)), far UV star formation rate (from -3.01 to -0.7 log(M$_\odot$ yr$^{-1}$)), and \hi mass (from 7.00 to 9.21 log(M$_\odot$)). This sample of 26 galaxies was selected to explore further the differences between global and local turbulence properties, and the impact of galactic properties on the feedback timescale. Section \ref{obs_c5} discusses the data used in this study from the Very Large Array (VLA\footnote{The VLA is operated by the NRAO, which is a facility of the National Science Foundation operated under cooperative agreement by Associated Universities, Inc.}), \textit{Hubble Space Telescope (HST)}, and WIYN\footnote{The WIYN Observatory is a joint facility of the NSF's National Optical-Infrared Astronomy Research Laboratory, Indiana University, the University of Wisconsin-Madison, Pennsylvania State University, the University of Missouri, the University of California-Irvine, and Purdue University. } 3.5m telescope, and Section \ref{Methods_c5} summarizes the methods detailed in Paper I and II for determining the SFHs and measuring the turbulence of the atomic and ionized gas.  Section \ref{halpha_res_c5} presents the H$\alpha$ results, Sections \ref{local_time_c5} and \ref{sec:equal} present the results for the \hi on the 400 pc scale, and Section \ref{sec:discussion_ch5} discusses the implications of these results.  Section \ref{global_time_c5} presents the global timescale results. Section \ref{conclusions_c5} summarizes the results and conclusions.

The SFHs were derived from observations of resolved stellar populations taken by \textit{HST} with either the Advanced Camera for Surveys instrument (\citealt{ACS}) or the Wide Field Planetary Camera 2 instrument (\citealt{WFPC2}).  Details of the observations are listed in Table  \ref{table:HST_obs_ch5}.  The ACS observations (202"$\times$202" field of view,  pixel scale of 0.05" pixel$^{-1}$) were taken with the camera's F814W I filter and at least one of the F606W V filter, F555W V filter, or F475W g filter. The WFPC2 observations were taken with the F814W I filter and either the F606W V filter or F555W V filter.  The WFPC2 instrument has three 800$\times$800 pixel wide field CCDs, with a 0.1" pixel $^{-1}$ pixel scale, and a 800$\times$800 pixel planetary camera CCD with a 0.05" pixel $^{-1}$ pixel scale. 

The optical imaging was processed in an identical manner to STARBIRDS \citep{McQuinn15a} and to match the processing in Paper I and II. A summary of the data reduction is provided here and the reader is referred to \cite{McQuinn10a} for a detailed description. Photometry was performed with the software DOLPHOT, optimized for the ACS and WFPC2 instruments, on the pipeline processed, charge transfer efficiency corrected images \citep{Dolphin00,Dolphot}. The photometry was filtered to include well-recovered point sources with the same quality cuts on signal-to-noise-ratios, crowding conditions, and sharpness parameters as applied in STARBIRDS. Artificial star tests were run on the individual images to measure the completeness of the stellar catalogs. As the derivation of the SFHs require a well-measured completeness function, $\sim5-6$ million artificial star tests were ran over each field of view, ensuring sufficient numbers of stars per individual region in the analysis.  

 %These estimates range from twice the disk scale heights of the galaxies (200-600 pc for dwarf galaxies measured in \cite{Patra20,Bacchini20b}), to an estimated driving scale of 2 kpc, (which is supported by \cite{Chepurnov15} who determined a 2.3 kpc turbulence driving scale from the velocity power spectrum of the SMC) and driving scales as large as 6 kpc have been predicted in simulations of dwarf galaxies \citep{Dib05}.  
 
 
%a clear correlation was evident across between the star formation at a specific time and nearly all \hi turbulence measures --100–200 Myr in Paper I for four low-mass galaxies, and in Paper II for Holmberg II.    
%In Papers I and II, a clear correlation was evident across between the star formation at a specific time and nearly all \hi turbulence measures --100–200 Myr in Paper I for four low-mass galaxies, and 70–140 Myr in Paper II for Holmberg II.  

%For the total sample, a large portion of the regions are located towards the outskirts of the galaxies. These regions have lower \hi column densities and historically have less star formation. Additionally, such regions tend to be the same regions with low current velocity dispersions. These regions can be seen on the outskirts of galaxies in Figures \ref{07843_frame} through \ref{92403_frame}. The analysis presented in the previous papers did not include significant numbers of regions in the outskirts of galaxies. In \LCHI, regions were required to have $>$50 blue stars and this blue star cut excluded the outer regions with low current star formation rates and gas masses.  In \LCHII, the HST footprint for Holmberg II does not cover the outer \hi extent of the galaxy. To illustrate the issue, in Figure \ref{sfrvhi_8.7} there is a large clustering of points with low star formation rates between 500 Myr to 14 Gyr ago and with velocity dispersions $\leq$15 km/s. This clustering appears to drive the possible correlation between the \hi velocity dispersions and the SFR in the oldest time bin. A reanalysis of the total sample with the blue star cuts in Sections \ref{blue_anal} removes many of these outer regions and shifts the peak of the correlation timescale. 


%Due to the lack of a clear correlation timescale between the SFHs and the velocity dispersions, the full sample of galaxies was re-analyzed focusing on the regions with indications of recent star formation activity.  As discussed in Paper I, the proof-of-concept analysis of four galaxies only included regions if they contained at least 50 young stars to ensure well-constrained recent SFHs.  However, these cuts were found to remove large numbers of regions of interest with star formation in the past 500 Myr. The subsequent analysis of Holmberg II discussed in Paper II did not include this cut. For the full sample, not making a cut results in the inclusion of many regions with low stellar mass, low \hi mass, and low velocity dispersion.  For some galaxies, imposing the cuts removes $\sim$10\% of the regions, with a negligible impact on the final analysis. For Holmberg II, the cut removes 13 out of 125 regions, and has no impact on the results.  However, for IC 2574, this cut removes nearly half the regions, going from 236 to 126 regions.   For the full sample 556 regions include the minimum number of blue stars. % The differences in the regions' SFHs can be seen in in Figures \ref{5666_SFH} and \ref{5666_SFH_blue}. The blue star cut removes many regions with high \hi velocity dispersions, as the blue star cut removes a prominent area of high velocity dispersion in the South of the galaxy (see Figure \ref{56663_frame}), as well as other smaller areas of high velocity dispersion. 
